That Doesn't Go There: Attacks on Shared State in Multi-User Augmented Reality Applications

Augmented Reality (AR) is expected to become a pervasive component in enabling shared virtual experiences. In order to facilitate collaboration among multiple users, it is crucial for multi-user AR applications to establish a consensus on the "shared state" of the virtual world and its augmentations, through which they interact within augmented reality spaces. Current methods to create and access shared state collect sensor data from devices (e.g., camera images), process them, and integrate them into the shared state. However, this process introduces new vulnerabilities and opportunities for attacks. Maliciously writing false data to "poison" the shared state is a major concern for the security of the downstream victims that depend on it. Another type of vulnerability arises when reading the shared state; by providing false inputs, an attacker can view hologram augmentations at locations they are not allowed to access. In this work, we demonstrate a series of novel attacks on multiple AR frameworks with shared states, focusing on three publicly-accessible frameworks. We show that these frameworks, while using different underlying implementations, scopes, and mechanisms to read from and write to the shared state, have shared vulnerability to a unified threat model. Our evaluation of these state-of-art AR applications demonstrates reliable attacks both on updating and accessing shared state across the different systems. To defend against such threats, we discuss a number of potential mitigation strategies that can help enhance the security of multi-user AR applications.

==> review.tex <==
%\fontsize{12}{12}\timesroman

\section*{Revision Details and Response}
\label{sec:reviews}
We thank the reviewers for their helpful feedback and the detailed revision requests provided for our manuscript. We have addressed each revision request, which we believe significantly improved the paper. Below, we outline our responses to the specific revision requests.  %We also made revisions suggested in the body of the reviews and therefore go over the review comments and the changes we made in response to them.

In the revised version of the manuscript, the major changes are highlighted in \revision{\textbf{blue text}}, alongside other smaller changes to improve clarity and readability. %The responses to the itemized review comments have been compiled as appendices, with each response distinctly marked in \green{\textbf{Green}} for ease of reference.
We welcome any additional suggestions regarding the revisions that will help us further improve the paper. %Thank you for your kind consideration of this manuscript. 


\subsection*{Revision requests}
\label{sec:revision_requests}
The revision request had 9 items, listed below with responses.\\

\noindent \textbf{1.} \textit{Clarify the fact that experiments did not impact users and findings were disclosed.}

\green{Thank you for raising this important concern. We performed all experiments either in sandboxes or in our own local sessions without external users: no public users were affected by our experiments. We added clarification of ethical considerations to the description of all three attack scenarios in \textbf{Sections ~\ref{sec:cloudanchor}, \ref{sec:geospatial}, and \ref{sec:mapillary}}.


We disclosed our findings to Google and Meta with respect to their AR frameworks. We added a paragraph about disclosures and ethics at the end of \textbf{Section~\ref{sec:intro}}. 
\\}

\noindent \textbf{2.} \textit{Clarify assumptions about attack preconditions / clarify the threat model.}

\green{We added clarification of the assumptions and preconditions for both the read attack and write attack in \textbf{Section~\ref{sec:threat}}.
For the read attack, this includes an API credential that is commonly hardcoded into the app (\eg when downloaded from the app store), as well as a room code that can be guessed through brute force. For the write attack, this includes images of the target location where the hologram is to be written.
\\}

\noindent \textbf{3.} \textit{Clarify that the attack methodology is not new, and the novelty lies in applying/adapting existing techniques to a new domain (AR).}

\green{We clarified that the mechanisms we use in the attack, such as image and GPS spoofing, are known and that our contribution is in showing how to leverage these attacks in multi-user AR application settings. Please see the end of the Introduction  \textbf{(Section~\ref{sec:intro}}).\\}

\noindent \textbf{4.} \textit{Provide better examples (context) that can clarify the practicability and consequences of the attacks.}

\green{Thank you for this suggestion. To address this request, in the revised paper, we highlight a number of examples throughout and describe their consequences.
In the construction worker attack scenario in the Introduction, later illustrated in \textbf{Section~\ref{sec:mapillary}}, an attacker can cause a construction worker to dig in dangerous locations.
In the private whiteboard example in \textbf{Section~\ref{sec:taxonomy}}, the attacker can gain access to private information.
In the scavenger hunt example in \textbf{Section~\ref{sec:geospatial}}, the attacker can cheat in the game.
We have demonstrated these attacks on commercial systems and therefore believe they are practical under the assumptions necessary for their success described in the threat model (\textbf{Section~\ref{sec:threat}}).\\}

\noindent \textbf{5.} \textit{Justify/show/evaluate defense mechanisms to detect proposed attacks, e.g., the use of depth sensors for 2D spoofing attacks.}

\green{Thank you for this excellent suggestion. The revision presents a proposed mitigation leveraging multi-modal sensors, including depth and visible light cameras, on an AR device (the Hololens 2).   
% In normal scenarios the defense performs well (over 90\% F1-score), while in challenging scenarios that include display panels, it achieves an F1-score of 79.35\%).  
The code and datasets for the defense are available at the following anonymous website: \url{https://sites.google.com/view/multi-ar-defense}. A new paragraph in \textbf{Section~\ref{sec:mitigations}} of the manuscript describes our experimental setup and the results evaluating the defense.\\}

\noindent \textbf{6.} \textit{Provide more technical details and evaluation details.}

\green{Thank you for this suggestion.
We have conducted additional experiments to understand the behavior of a benign baseline, as well as the impact of distance on attack success in Scenario A.
These results are shown in \textbf{Fig.~\ref{fig:RR_distance_result}} and \textbf{Fig.~\ref{fig:RW_distance_result}} and discussed in \textbf{Section~\ref{sec:cloudanchor-eval} and \textbf{Appendix~\ref{app:cloudanchor}}}.
 %We have incorporated a new
 %\textbf{Appendix~\ref{sec:appendix}} to provide more complete technical and evaluation details. 
 %Specifically, to enhance the understanding of Scenario A, two new figures, \textbf{Fig.\ref{fig:RR_distance_result}} and \textbf{Fig.\ref{fig:RW_distance_result}}, have been added in \textbf{Appendix~\ref{sec:scenario_A_results}} to present additional evaluation results. 
 We also added additional details on the experimental procedures for all three attack scenarios in \textbf{Appendix~\ref{app:experiment_procedure}}.
 This includes \textbf{Fig.~\ref{fig:arcore_environments}} and \textbf{Fig.~\ref{fig:geospatialexample}} to illustrate the indoor and outdoor scenes tested in Scenarios A and B. 
% \yicheng{Need examples of cloud anchor indoor and outdoor scenes.}
\\}

\noindent \textbf{7.} \textit{Address spelling and grammar issues throughout.}

\green{We have carefully revised the manuscript to improve the clarity of figures and tables, fix typos and remove repeated references.\\}

\noindent \textbf{8.} \textit{Improve the organization and presentation of the paper.}

\green{We responded to the reviewer's suggestions regarding organization and presentation. Specifically, we placed \textbf{Table~\ref{ttable3}} in \textbf{Section~\ref{sec:remote-read-eval}}, \textbf{Table~\ref{tab:remote-write-clutter}} in \textbf{Section~\ref{sec:cloudanchor-write-eval}} and \textbf{Table~\ref{ttable2}} in \textbf{Section~\ref{sec:trigger_remote_read_eval}} respectively to make sure tables are in their related subsections as suggested by reviewer D. We corrected typos and removed repeated references and capitalization of Read/Write as pointed out by reviewer C and D. We also made other changes to improve organization of the paper. For instance, we added a new \textbf{Appendix~\ref{app:cloudanchor}} to provide a number of examples of scenes where we conducted our attacks (\textbf{Fig.~\ref{fig:arcore_environments}} and \textbf{Fig.~\ref{fig:geospatialexample}}) to help better understand our attacks. We rewrote parts of \textbf{Section~\ref{sec:threat}} (threat model) and summarized the attacker's goals in each scenario.\\}



\noindent \textbf{9.} \textit{Clarify all points and make changes promised in your rebuttal.}


\green{In the remainder of this response letter, we go over the changes promised in the rebuttal and describe how we addressed them. \\}



\subsection*{Promised changes in the rebuttal}

% \subsubsection*{}

In this section, we review all the changes we promised in the rebuttal and detail the changes we made in the manuscript to satisfy them. \\

\noindent \textbf{1.} \textit{ We will revise the manuscript carefully to improve figure/table clarity and catch typos and repeated references.}

\green{This change was brought up in response to concerns by reviewer C and reviewer D. We revised the manuscript carefully to improve the figure and table clarity. We proofread the manuscript to find and correct typos, repeated references, and other issues, such as inconsistent capitalization of Read/Write. Please see the response to \textbf{Revision requests 8} for more details. \\}


\noindent \textbf{2.} \textit{We will add an evaluation for defense mechanisms involving depth sensors (like LiDAR on iPhone) to reject spoofed 2D images.}

\green{Reviewers B, C, and D raised concerns about the absence of a concrete evaluated mitigation. We added an evaluation for defense mechanisms involving depth sensors to reject spoofed 2D images and prevent remote reads and writes from taking place. Please find more details under the response to \textbf{Revision requests 5} above.\\}

\noindent \textbf{3.} \textit{We will weaken the claims of the AR taxonomy contribution if the reviewers prefer.}

\green{We thank Reviewer B for pointing out this concern. We weakened the claims of the AR taxonomy contribution. We also revised the list of contributions at the end of \textbf{Section~\ref{sec:intro}}. Please refer to our response to \textbf{Revision request 3} for more details.\\}


\noindent \textbf{4.} \textit{Benign AR baselines generally have a high success rate. We will add results to show this in a revision, as a function of distance for Scenarios A and B.}

\green{Reviewer D raised a question about benign AR baseline, to which we responded promising to add results to support this answer. We conducted additional experiments and found that the benign baseline (no attack) succeeds at reading or writing holograms essentially 100\% of the time for both Scenarios A and B. We added evaluation results in \textbf{Section~\ref{sec:cloudanchor-eval}} and \textbf{Appendix~\ref{sec:scenario_A_results}} to showcase this (specifically, \textbf{Fig.~\ref{fig:RR_distance_result}} and \textbf{Fig.~\ref{fig:RW_distance_result}}). Furthermore, we conducted tests on remote read and remote write attacks from varying distances, which is also shown in these figures.\\}

 
\noindent \textbf{5.} \textit{Most algorithms used in Scenarios A and B are closed-source. We will add additional background to describe the API calls and pictures/details of the attack environments.}

\green{The concern is raised by Reviewer D. We added a new \textbf{Appendix~\ref{app:experiment_procedure}} to provide more complete information on the experimental methodology, API calls, and pictures of the attack environments. Please check our responses in \textbf{Revision request 6}.}

%In the remainder of this response, we will provide detailed information about the additional changes made to the manuscript in response to these reviews.
%\yicheng{Add rebuttal and show a checklist for each point.}
% This section will review all the points and detail the changes we committed to in our rebuttal. We first go through 5 common concerns from reviewers. Then, we detail additional changes we made in response to each reviewer.

\iffalse
\subsubsection*{Common concerns}


\noindent \textbf{a.} \textit{Threat models (RevB, RevE).}

\green{We clarified the assumptions and provided examples for the three attack scenarios. Please check responses to \textbf{Revision requests 3 and 4} for details. \\}


\noindent \textbf{b.} \textit{Ethical considerations/attacks affecting others (RevA, RevC).}

\green{We revised the paper as suggested in the first revision request. Please check responses \textbf{Revision request 1} above.\\}


\noindent \textbf{c.} \textit{Attack novelty (RevB, RevE).}

\green{We revised the claims in the list of contributions towards the end of \textbf{Section~\ref{sec:intro}} to emphasize that GPS and image spoofing are known, and that our contributions are around leveraging them in the context of shared state for multi-user AR, to cause adverse downstream effects on victims. Please see the response to \textbf{Revision request 3} above for more details.\\}


\noindent \textbf{d.} \textit{Writing and organization (RevC, RevD).}


\green{We revised the manuscript carefully to improve the figure and table clarity. Please see response to \textbf{Revision requests 8} for more details. \\}

\noindent \textbf{e.} \textit{Mitigations (RevB, RevC, RevD)}


\green{In response to the fifth revision request, we added an evaluation for defense mechanisms involving depth sensors to reject spoofed 2D images and prevent remote reads and writes from taking place. Please find more details under the response to \textbf{Revision requests 5} above.\\ }


\subsubsection*{Rebuttal response to Review 218A}
\noindent \textbf{a.} \textit{I was confused by the discussion of the use of OpenSFM rather than Mapillary itself. How close is what was tested to how Mapillary actually works?}

\green{Thank you for raising this question.
We first demonstrated the attacker's write to Mapillary's servers is successful.
OpenSFM is simply used to visualize the effect of the attack from the victim's side, since we do not have access to the raw data on Mapillary servers.
Indeed, OpenSFM is one of the core components of the Mapillary pipeline used for 3D reconstruction as stated on their website\footnote{\url{https://www.mapillary.com/technology?locale=en_US}}, and based on our conversations with Mapillary engineers. %Specifically, Mapillary uses OpenSFM for 3D reconstruction while using other proprietary algorithms for privacy blurring, traffic sign recognition, etc. 
However, it is important to note that the Mapillary pipeline is closed and includes additional unreleased components. These include features such as filtering images with inappropriate content and blurring human faces, which are integral to promoting privacy. These did not affect our results because we verified that our images were successfully uploaded to Mapillary's servers during the write attack, passing through such filters. We added some text to \textbf{Section~\ref{sec:mapillaryswap}} to clarify this.
}

\subsubsection*{Review 218B}

\noindent \textbf{a.} \textit{Unclear evaluation in Section 5.2.}

\green{Thank you for this concern. Please see our sixth response in \textbf{Revision request 6}. We included detailed experimental procedures for all three attack scenarios, which have been documented in \textbf{Appendix~\ref{app:experiment_procedure}}. \\
}

\noindent \textbf{b.} \textit{Contribution to AR frameworks taxonomy.}

\green{We weaken the claims of the AR taxonomy contribution as in the third revision request. We revised the list of contributions at the end of \textbf{Section~\ref{sec:intro}}. Please refer our responses in \textbf{Revision request 3}.\\
}


\subsubsection*{Review 218C}

\noindent \textbf{a.} \textit{Motivation for the AR frameworks and Scenario A attack sub-types.}

\green{Thank you for pointing this out.
We added the motivation for those particular AR frameworks in the Introduction \textbf{(Section~\ref{sec:intro})} and the Scenario A attack sub-types in \textbf{Section~\ref{sec:cloudanchor-method}}.
In brief, we focus on Meta and Google APIs because they are major commercial players in the AR ecosystem.
The three attack sub-types in Scenario A are read, write, and triggered write. We focus on read and write because they are fundamental primitives, and triggered write as a more advanced write.
Certainly, there may be more sub-types in the future, and we hope that our work can spur further investigations.
%We revised \textbf{Section~\ref{sec:threat}} by summarizing the attacker’s benefits in each scenario. Please check our responses in \textbf{Revision request 3}. Also, for scenario A attack sub-types, we provide a series of examples for these attacks in \textbf{Section~\ref{sec:threat}} as we describe in \textbf{Revision request 4} above.
%\jiasi{will work on this one to motivate why these frameworks and why the Scenario A sub-types}
%\textbf{Section~\ref{sec:cloudanchor-method}}
\\
}

\subsubsection*{Review 218D}

\noindent \textbf{a.} \textit{Benign baseline.}

\green{Thanks for your valuable suggestion. We conducted additional experiments and found that the benign baseline (no attack) succeeds at reading or writing holograms essentially 100\% of the time. We added evaluation results in \textbf{Section~\ref{sec:cloudanchor-eval}} and \textbf{Appendix~\ref{sec:scenario_A_results}} to showcase this (specifically, \textbf{Fig.~\ref{fig:RR_distance_result}} and \textbf{Fig.~\ref{fig:RW_distance_result}}). %The extended evaluations include adding a benign baseline for Scenario A. 
Furthermore, we conducted tests on remote read and remote write attacks from varying distances, which is also shown in these figures.\\
}

\noindent \textbf{b.} \textit{API and environment details.}

\green{%We added the additional background to describe the API calls and pictures/details of the attack environments.

We added a new \textbf{Appendix~\ref{app:experiment_procedure}} to provide more complete information on the experimental methodology, API calls, and pictures of the attack environments. Please check our responses in \textbf{Revision request 6}.
\jiasi{will work on this one to add API call details}\\
}

\subsubsection*{Review 218E}

\noindent \textbf{a.} \textit{Consequences of the attacks are unclear.}

\green{Thank you for this concern. We responded to this request in \textbf{Revision request 4}. \\


}
\fi

==> todo.tex <==
\section*{Revision To Do}

\revision{-add rebuttal wording where appropriate (carter)} \jiasi{Carter, I got through many of the bigger changes from the shepherd's list (see below). Could you go through the rest of the shepherd's list and the individual reviews to check for corrections? Let me know how far you get and I can pick up from there.}

\revision{-Clarify the fact that experiments did not impact users and findings were disclosed \carter{done,revised  A and B to be closer to rebuttal wording, C was already close, still need to confirm google disclosure}}
\jiasi{I revised, looks good. Confirm if we did Google disclosure.}


\revision{-Clarify assumptions about attack preconditions / clarify the threat model \carter{done, double checked}} \jiasi{revised and done}

\revision{-Clarify that the attack methodology is not new, and the novelty lies in applying/adapting existing techniques to a new domain (AR).\carter{done, double checked}} \jiasi{done 2}

\revision{-Provide better examples (context) that can clarify the practicability and consequences of the attacks. \jiasi{done, I found we already had many examples throughout (maybe the reviewer did not read carefully), I tried to highlight further}\carter{agreed}} 

\revision{-Justify/show/evaluate defense mechanisms to detect proposed attacks, e.g., the use of depth sensors for 2D spoofing attacks. \carter{Yichengs RGBD binary classifier can go here}} \yicheng{Done}

\revision{-Provide more technical details and evaluation details \carter{done for mappilary, will need help on the others (what devices? what image resolution, etc)}}
\jiasi{need to add methodology to Appendix and fill in various details throughout as mentioned by individual reviewers. Should we offer to release Mapillary scripts? Android apps are just the default ones, nothing to release}

\revision{-Address spelling and grammar issues throughout \carter{will do  in Jan}}


\revision{-Improve the organization and presentation of the paper \carter{will do  in Jan}}

\revision{-Clarify all points and make changes promised in your rebuttal}

\revision{-Remove capitalization of Read/Write} \yicheng{Done but needs double check.}
